DNNShield: Dynamic Randomized Model Sparsification, A Defense Against Adversarial Machine Learning

DNNs are known to be vulnerable to so-called adversarial attacks that manipulate inputs to cause incorrect results that can be beneficial to an attacker or damaging to the victim. Recent works have proposed approximate computation as a defense mechanism against machine learning attacks. We show that these approaches, while successful for a range of inputs, are insufficient to address stronger, high-confidence adversarial attacks. To address this, we propose DNNSHIELD, a hardware-accelerated defense that adapts the strength of the response to the confidence of the adversarial input. Our approach relies on dynamic and random sparsification of the DNN model to achieve inference approximation efficiently and with fine-grain control over the approximation error. DNNSHIELD uses the output distribution characteristics of sparsified inference compared to a dense reference to detect adversarial inputs. We show an adversarial detection rate of 86% when applied to VGG16 and 88% when applied to ResNet50, which exceeds the detection rate of the state of the art approaches, with a much lower overhead. We demonstrate a software/hardware-accelerated FPGA prototype, which reduces the performance impact of DNNSHIELD relative to software-only CPU and GPU implementations.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> threat.tex <==
\section{Threat Model}
\label{sec:threat}

We assume in this paper that the adversary has complete access to the DNN model, including the output prediction and logits, with full knowledge of the architecture and parameters, and is able to use this in a white-box manner. 
%%DAC remove
%We assume an adversary that is able to directly supply inputs to the ML classifier, such as in \cite{eykholt2018robust,pautov2019adversarial,raju2020blurnet} where attackers generate  visual  adversarial perturbations that are supposed to mimic real-world obstacles or create adversarial traffic signs to attack autonomous driving. 
We focus mainly on recent state-of-the-art optimization-based attacks--CW and EAD--since it has been demonstrated that all earlier attacks can be overcome utilizing other methods, such as adversarial training \cite{goodfellow2014explaining} or defensive distillation \cite{papernot2016distillation}, 
which could be used in combination with our approach. These attacks can increase their confidence without sacrificing too much distortion in the input image, which makes them resilient against fixed levels of noise. We also focused on Imagenet dataset as the best representation of high-resolution real-world images rather than small datasets like MNIST and Cifar. 
%Additionally, we verify our evaluation includes high confidence adversarial examples, as some previously proposed defenses were later shown to perform poorly under a more holistic treatment which included these inputs \cite{lu2018on}. 




